Magnetically Insulated Diode: Existence of Solutions and Complex Bifurcation. I

In order to avoid the electron oscillation of the cathode and enhance the work efficiency of a vacuum diode, an approach for analyzing the solutions and complex bifurcation has been proposed and used to determine the optimal trajectory of electron motion of the vacuum diode. This work is focusing on the stationary self-consistent problem of magnetic insulation in a space-charge-limited vacuum diode, modeled by a singularly perturbed 1.5-dimensional Vlasov-Maxwell system. We focus on the insulated regime, characterized by the reflection of electrons back toward the cathode at a point $x^{*}.$ The analysis proceeds in two primary stages. First, the original Vlasov-Maxwell system is reduced to a nonlinear singular system of ordinary differential equations governing the electric and magnetic field potentials. Subsequently, this system is further reduced to a novel nonlinear singular ODE for an effective potential $\theta(x).$ The existence of non-negative solutions to this final equation is established on the interval $[0, x^{*})$, where $\theta(x)>0$. This is achieved by reformulating the associated initial value problem into a system of coupled nonlinear Fredholm integral equations and proving the existence of fixed points for the corresponding operators. The most significant and previously unexplored case occurs when $\theta(x)<0$ on the interval $(x^{*}, 1]$, which corresponds to the fully insulated diode. For this regime, we present a novel numerical analysis of complex solution bifurcations, examining their dependence on system parameters and boundary conditions. Bifurcation diagrams illustrating the solution $\theta(x)$ as a function of the free boundary $x^{*}$ is constructed, and the insulated diode spacing is determined.

==> Sections/Bifurcation_Subsections/Particular_Case.tex <==
\subsection{Particular Case $\hat{\beta}=\hat{k}$}

==> Sections/Boundary.tex <==
\section{Boundary value problem}
\subsection{Taylor Series Approximation}

Let us return to the equation (52) with condition (53) and derivative of effective potential  
$$
\theta'(x)= \pm[8j_{x}\theta^{3/2} + 8 j_{x}\theta^{1/2} + 2k_{1}\theta + k_{2}]^{1/2},                 \eqno(5.1)
$$
where $k_{1}, k_{2}=4\beta^{2}$ are constants which we need to define. Our idea is to approximate the right hand side of (5.1) by a quadratic polynomial in $\theta$ in  a Taylor series  around some value $\theta_{L}>0$. We define the real function approximation $f\in [0, \theta_{L}]$ 
$$
f(\theta)= \pm [8 j_{x} \theta^{1/2}(\theta+1) + 2k_{1}\theta + k_{2}]^{1/2}       \eqno(5.2)
$$
and calculate its two first derivatives with respect to variable $\theta$
$$
\begin{array}{l}
f'(\theta)=\big[2j_x\theta^{-1/2}\big(3\theta+1\big)+k_1\big]f^{-1},
\\
f''(\theta)=\big\{j_x\theta^{-3/2}\big(3\theta-1\big)-\big[2j_x\theta^{-1/2}\big(3\theta+1\big)+k_1\big]^2f^{-2}\big\}f^{-1}.
\end{array}                  \eqno(5.3)
$$
$f(\theta)\neq 0, \; \theta'(x)\neq 0, \;\; \theta'(0)=k_{2}^{1/2} = 2\beta>0$. It follows that $k_{2}$ is strictly positive and consequently the Child-Langmuir regime  does not work in this discussion. We introduce  notation
$$
\begin{array}{l}
f^{(\eta)}_L \equiv f^{(\eta)}(\theta_L), 
  \\
f^{(\eta)}_0 \equiv f^{(\eta)}(0),
\end{array}
\quad\quad \textrm{where }\eta=0,1,2,\textrm{ is  order of the derivative},\quad\quad\theta_L>0.  \eqno(5.4)
$$
We exclude values $\theta_{L}\leq 0$ since the derivatives (5.3) evaluated at $\theta = 0$ produce uncertainties. The Taylor expansion to second order $f(\theta)$ around $\theta_L$ it can be constructed as
$$
f(\theta)=\sum_{r=0}^{\infty}\frac{1}{r!}f^{(r)}_L(\theta-\theta_L)^r=f_L+f'_L(\theta-\theta_L)+\frac{1}{2}f''_L(\theta-\theta_L)^2+O\big(f_L^{-1}\big)
\approx\theta'(x).    \eqno(5.5)
$$
Then, the functions (5.2) - (5.3) can now take the approximate shape
$$
\begin{array}{l}
 f(\theta)\approx\frac{1}{2}f''_L(\theta-\theta_L)^2+f'_L(\theta-\theta_L)+f_L,
  \\
  \!f'(\theta)\approx f''_L(\theta-\theta_L)+f'_L, 
  \\
  \!\!f''(\theta)\approx f''_L.
\end{array}   \eqno(5.6)
$$
and
$$
\begin{array}{l}
  f_0\approx\frac{1}{2}\theta_L^2f''_L-\theta_Lf'_L+f_L\approx\pm k_2^{1/2}=\pm2\beta, 
  \\
  f'_0\approx-\theta_Lf''_L+f'_L, 
  \\
  \!f''_0\approx f''_L.
\end{array}                     \eqno(5.7)
$$
The decompositions $f'(\theta), \; f_{0}^{'}$ in (5.6), (5.7) reduce ODE (5.1) to the integrated form with solution 
$$
x\approx\int_0^{\theta}\dfrac{\textrm{d}\tilde{\theta}}{f(\tilde{\theta})}=
\dfrac{2}{R_L}\bigg[\arctan\dfrac{f'(\theta)}{R_L}-\arctan\dfrac{f'_0}{R_L}\bigg],          \eqno(5.8)
$$
\bigskip\noindent where we have defined the amount 
$$
R_L\equiv R(\theta_L)=\pm\big\{2f_Lf''_L-(f'_L)^2\big\}^{1/2},          \eqno(5.9)
$$
We write (5.8) in terms of variable $\theta(x)$
$$
\theta(x)\approx\dfrac{R_L}{f''_0}\tan\bigg[\dfrac{R_L}{2}x+\arctan\dfrac{f'_0}{R_L}\bigg]-\dfrac{f'_0}{f''_0},       \eqno(5.10)
$$
or 
$$
\theta(x)\approx A\tan(Bx+C)+D,          \eqno(5.11)
$$
where
$$
  A=\frac{R_L}{f''_0}, \quad\quad\quad
  B=\frac{R_L}{2}, \quad\quad\quad
  C=\arctan\frac{f'_0}{R_L}, \quad\quad\quad
  D=-\frac{f'_0}{f''_0}.                       \eqno(5.12)
$$
Note that the constant $D$ can also be written as $D= \theta_{L} - \frac{f'(\theta_{L})}{f''(\theta_{L})}$ , which it is precisely the standard Newton-Raphson algorithm $x_{i+1}= x_{i}- \frac{F(x_{i})}{F'(x_{i})}$ for all $i\geq 0$, with $x_{i}= \theta_{L}$, $x_{i+1}=D, F=f'$ and whose successive iteration it is often used to locate the zeros of a numerically function $f'$ with real variable $\theta_{L}$.

\subsubsection{Own Requirements of Effective Potential. First Requirement: $f(\theta)\neq 0$}.

We introduce the following notations 
$$
K_1\equiv\dfrac{k_1}{j_x},\quad\quad\quad K_2\equiv\dfrac{k_2}{j_x}>0, \eqno(5.13)
$$
From (5.6) we obtain the first condition
$$
K_2\neq-2\theta_L^{1/2}\big[\theta_L^{1/2}K_1+4(\theta_L+1)\big].  \eqno(5.14)
$$

\subsubsection{Second Requirement: \;$f^{''}_{0}\neq 0$}

Second derivative in (5.6) gives 
$$
K_2\neq\theta_L^{1/2}\bigg[\dfrac{(\theta_L^{1/2}K_1+3\theta_L+3)^2}{3\theta_L-1}+\theta_L-3\bigg],\quad\quad\theta_L\neq\frac{1}{3}.  \eqno(5.15)
$$

\subsubsection{Third Requirement:\;$\theta\neq \pm \infty$}

This requirement directly involves the domain $x\in [0, 1]$ and it refers to those values for which the effective potential is indeterminate. When $\theta(x)$ a tangent function, their asymptotes occur at odd intervals of $\pi/2$ of the argument as well, because of (5.10) we conclude that
$$
x\neq\dfrac{(2l+1)\pi}{R_L}-\dfrac{2}{R_L}\arctan\dfrac{f'_0}{R_L},\quad\quad\textrm{for all }l\in\mathbb{Z},   \eqno(5.16)
$$
and we apply (5.2), (5.3), (5.7) to write functions $R_{L}$, $f_{0}^{'}$ as
$$
\begin{array}{l}
\!\!R_L=\pm j_x^{1/2}\big\{2\theta_L^{-3/2}(3\theta_L-1)-3j_xf_L^{-2}[2\theta_L^{-1/2}(3\theta_L+1)+K_1]^2\big\}^{1/2}\neq0,
\\
f'_0\approx\pm j_x^2f_L^{-3}\big\{j_x^{-1}f_L^{2}[3\theta_L^{-1/2}(\theta_L+1)+K_1]+\theta_L[2\theta_L^{-1/2}(3\theta_L+1)+K_1]^2\big\}.
\end{array}      \eqno(5.17)
$$

\subsubsection{Fourth Requirement: ${\rm arg}\{R_{L}\}>0$}
$$
f_Lf''_L>\frac{1}{2}(f'_L)^2.          \eqno(5.18)
$$
$$
K_1=-2\theta_L^{-1/2}(3\theta_L+1)\leq-4\sqrt{3}.
$$
We obtain from (5.17)
$$
K_2>z_0+z_1K_1+z_2K_1^2\equiv Z(\theta_L;K_1),              \eqno(5.19)
$$
where the coefficients $z_{i}= z_{i}(\theta_{L})$ are given by
$$
  z_0=\frac{2\theta_L^{1/2}(15\theta_L^2+10\theta_L+7)}{3\theta_L-1},
  \quad\quad\quad
  z_1=\frac{4\theta_L(3\theta_L+2)}{3\theta_L-1}, 
  \quad\quad\quad
  z_2=\frac{3\theta_L^{3/2}}{2(3\theta_L-1)}.
$$
\subsection{Boundary Conditions}

Before the consideration of magneto insulated diode, we will consider the influence of boundary conditions
$$
\theta(0)=0, \;\; \theta(1)= [1+ \varphi_{L}]^2 - 1 - a_{L}^{2}\equiv \theta_{L}, \;\; \theta'(0)=2\beta\geq 0.          \eqno(5.20)
$$
These conditions are of crucial importance in what follows. We calculate the derivative of the effective potential (5.10)
$$
\theta'(x)\approx AB\sec^2(Bx+C)=\frac{B}{A}\big[A^2+(\theta-D)^2\big], \eqno(5.21)
$$
where $A$, $B$, $C$ and $D$ are defined by (5.12).

\subsubsection{First Condition: $\theta (0) \approx 0$}

We apply the first condition in (5.20) to the function (5.10)
$$
\tan C\approx-\frac{D}{A},           \eqno(5.22)
$$
we  eliminate the constant $C$ of the effective potential for
$$
\theta(x)=\dfrac{A^2+D^2}{A\cot Bx+D},            \eqno(5.23)
$$
or we have with (5.7), (5.9), (5.12)
$$
\theta(x)=\dfrac{2f_0}{R_0\cot(\frac{R_0x}{2})-f'_0},      \eqno(5.24)
$$
with
$$
R_0=\pm\big\{2f_0f''_0-(f'_0)^2\big\}^{1/2}=R_L.                 \eqno(5.25)
$$
To avoid uncertainties, the denominator in (5.23) must be non-zero which leads to 
$$
x\neq\dfrac{2}{R_0}\arctan\dfrac{R_0}{f'_0},\quad\quad f'_0\neq0,  \eqno(5.26)
$$
We can deduce by the second equation in (5.17) that
$$
K_2\neq-\theta_L^{1/2}\Bigg[\dfrac{3\theta_LK_1^2+2\theta_L^{1/2}(13\theta_L+9)K_1+4(15\theta_L^2+18\theta_L+7)}{\theta_L^{1/2} K_1+3(\theta_L+1)}\Bigg].\eqno(5.27)
$$

\subsubsection{Second Condition: $\theta(1)\approx \theta_{L}.$}

 We combine second boundary condition  with  condition (5.20) for
 $$
\tan B\approx\dfrac{\theta_LA}{A^2+D^2-\theta_LD}.  \eqno(5.28)
$$
We define the amount using (5.2), (5.3)
$$
\Omega\equiv\frac{2\theta_L}{2f_L-\theta_Lf'_L}=\dfrac{2j_x^{-1}\theta_Lf_L}{
3\theta_LK_1+2K_2+2\theta_L^{1/2}(5\theta_L+7)}\neq0,       \eqno(5.29)
$$
We transform (5.27) with (5.7), (5.9), (5.12) in  
$$
\tan B-\Omega B\approx0,                           \eqno(5.30)
$$
which requires 
$$
K_2\neq-
\frac{3}{2}\theta_LK_1-\theta_L^{1/2}(5\theta_L+7).            \eqno(5.31)
$$
The left side of (5.29) can not be indefinite, then the argument of the tangent is
$$
R_L\neq(2l+1)\pi,\quad\quad\textrm{for all }l\in\mathbb{Z}.       \eqno(5.32)
$$

\subsubsection{Third Condition: $\theta'(0)\approx 2\beta >0$.}

The last condition in (5.20) allows us to demonstrate the relationship 
$$
k_{2}= 4\beta^{2}\geq 0.                      \eqno(5.33)
$$
We obtain from (5.12), (5.21), (5.24)
$$
2\beta\approx\dfrac{B}{A}\big[A^2+D^2\big]=f_0,        \eqno(5.34)
$$
Comparison with the first relationship in (5.7) leads to (5.33). We couple the first relationship (5.7) with the formulas (5.2) - (5.3) evaluated in $\theta=\theta_{L}$ and scaled quantities (5.13) to develop trinomial
$$
\big(2f_L-2\theta_Lf'_L+\theta_L^2f''_L\big)^2-4j_xK_2\approx 0.
$$
Multiplying  last expression by $j_x^{-4}f_L^6$ and conducting extensive algebraic treatment, we will obtain an independent expression of $j_x$ with the form
$$
Q(\theta_L;K_1,K_2)=q_0+q_1K_2+q_2K_2^2+q_3K_2^3\approx 0, \eqno(5.35)
$$
which emerges here as the second most important result of this research functions $q_{i}= q_{i}(\theta_{L}; K_{1}), \; i=0,1,2,3,$ given by polynomials
$$
\begin{array}{l}
  q_0=\theta_L^2\big[3\theta_LK_1^2+2\theta_L^{1/2}(17+9\theta_L)K_1+4(21+30\theta_L+5\theta_L^2)\big]^2,
     \\
  q_1=4\theta_L^3K_1^3+6\theta_L^{5/2}(31-5\theta_L)K_1^2+
  4\theta_L^2(327+226\theta_L-117\theta_L^2)K_1
  \\+
  8\theta_L^{3/2}(311+525\theta_L+57\theta_L^2-141\theta_L^3), 
  \\
  q_2=4\theta_L^{3/2}(19-9\theta_L)K_1+
  3\theta_L(99+62\theta_L-53\theta_L^2),
  \end{array}                                  \eqno(5.36)
$$

\subsection{Magnetically insulated  Diode}

We introduce  the condition for magnetic insulation
$$
\theta(x)<0                          \eqno(5.37)
$$
Solution (5.10) gives
$$
R_{L}x<0.
$$
Since $x$ can only take positive values, it not only excludes condition $x = 0$ but also exerts a strong constraint on $R_L$ forcing it to be negative. This means that for magnetic isolation should
be considered in (5.9) the root
$$
-\big\{2f_Lf''_L-(f'_L)^2\big\}^{1/2}<0.               \eqno(5.38)
$$
Thus, to describe a magnetically insulated plane diode, hereinafter should be considered only negative in all calculations involving the number $R_L$. 

\subsection{Case i: $K_{1}=0, K_{2}>0$.}

From (5.19) we have
$$
K_2>\dfrac{2\theta_L^{1/2}(15\theta_L^2+10\theta_L+7)}{3\theta_L-1}=Z(\theta_L;0)\equiv Z_L^{(0)}.          \eqno(5.39)
$$
In this case, $K_{1}=0$, the coefficients $q_{i}=q_{i}(\theta_{L}; 0), \; i=0,1,2,3$ are
$$
\begin{array}{l}
  q_0=16\theta_L^2(21+30\theta_L+5\theta_L^2)^2,
     \\
  q_1=8\theta_L^{3/2}(311+525\theta_L+57\theta_L^2-141\theta_L^3), 
  \\
  q_2=3\theta_L(99+62\theta_L-53\theta_L^2),
  \\
  q_3=4\theta_L^{1/2}(3-\theta_L).
\end{array}
$$

\subsection{Case ii: $K_{1}=K_{2}=K>0.$}

The condition (5.19) now takes the quadratic form
$$
\zeta\equiv\sigma_0+\sigma_1K+\sigma_2K^2<0,      \eqno(5.40)
$$
where coefficients $\sigma_i=\sigma_i(\theta_L)$ are given
$$
\begin{array}{l}
  \sigma_0=4\theta_L^{1/2}(15\theta_L^2+10\theta_L+7),
  \\
  \sigma_1=2(12\theta_L^2+5\theta_L+1), 
  \\
  \sigma_2=3\theta_L^{3/2}.
\end{array}                              \eqno(5.41)
$$
Since $\theta_L$ is positive, $\sigma_i$ always be positive so that the family of curves $\zeta(\theta_L;K)$ draw parabolas concave upward in the plane. This suggests that each $\theta_L$ it is associated a parable with an absolute minimum $\zeta_{\textrm{min}}=\zeta(K_{\textrm{min}})$ where $K_{\textrm{min}}$ y $\zeta_{\textrm{min}}$ are functions of $\theta_L$ given by\footnote{It is clear that $K_{\textrm{min}}$ it must be bad for not conflict with (2.55). For its part, $\zeta_{\textrm{min}}$ It is positive and inversely proportional to $\theta_L$ when $0<\theta_L\leq1/3$ and it is negative and proportional to $\theta_L>1/3$. Height $K_{\textrm{min}}=-{92\sqrt{3}}/{27}\simeq5_{\cdot}9$ occurs when $\theta_L=3/4$.}
$$
\begin{array}{l}
\!\!  K_{\textrm{min}}(\theta_L)=-\frac{12\theta_L^2+5\theta_L+1}{3\theta_L^{3/2}}\leq-\frac{92\sqrt{3}}{27},
  \\
  \zeta_{\textrm{min}}(\theta_L)=\frac{1+10\theta_L-35\theta_L^2-36\theta_L^4}{3\theta_L^{3/2}}.
  \end{array}      \eqno(5.42)
$$
